Conditioning Accept-Desirability models in the context of AGM-like belief change

We discuss conditionalisation for Accept-Desirability models in an abstract decision-making framework, where uncertain rewards live in a general linear space, and events are special projection operators on that linear space. This abstract setting allows us to unify classical and quantum probabilities, and extend them to an imprecise probabilities context. We introduce a new conditioning rule for our Accept-Desirability models, based on the idea that observing an event introduces new indifferences between options. We associate a belief revision operator with our conditioning rule, and investigate which of the AGM axioms for belief revision still hold in our more general framework. We investigate two interesting special cases where all of these axioms are shown to still hold: classical propositional logic and full conditional probabilities.

==> config.tex <==
\usepackage[charter]{mathdesign}
\usepackage[nottoc,notlot,notlof]{tocbibind}
\usepackage{tikz}
\usetikzlibrary{datavisualization}
\usetikzlibrary{patterns}
\usetikzlibrary{math}
\usetikzlibrary{positioning}
\tikzset{
    clip even odd rule/.code={\pgfseteorule}, % Credit to Andrew Stacey
    invclip/.style={
        clip,insert path=
            [clip even odd rule]{
                [reset cm](-\maxdimen,-\maxdimen)rectangle(\maxdimen,\maxdimen)
            }
    }
}
\usepackage{nicefrac}
\usepackage[utf8]{inputenc}

\usepackage[
backend=biber,
style=numeric,
sorting=none
]{biblatex}

\usepackage{textcomp}
\usepackage{amsfonts}
\usepackage{gensymb}
\usepackage{amsmath}
% \usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bbm}

\usepackage{mathrsfs}
\usepackage{thmtools}
\usepackage{xparse}
\usepackage{caption}
\usepackage{mathtools}

\usepackage{parskip}
\usepackage{titlesec}


\usepackage{newfloat}
\usepackage[dvipsnames]{xcolor}
\definecolor{definecolour}{RGB}{45,125,162}
% \usepackage{mathabx}
\usepackage{multicol}
\usepackage{graphicx}

\usepackage{hyperref}
\makeatletter
\def\namedlabel#1#2{\begingroup
    #2%
    \def\@currentlabel{#2}%
    \phantomsection\label{#1}\endgroup
}
\makeatother
\usepackage{caption}
\usepackage{enumitem}
\usepackage{floatrow}

%%%%%%%%%%%
% Margins %
%%%%%%%%%%%
\usepackage[inner=2.5cm,outer=2.5cm,top=3cm,bottom=3cm]{geometry} % Digital
%\usepackage[inner=3.4cm,outer=1.6cm,top=3cm,bottom=3cm]{geometry} % Print

\usepackage[final]{pdfpages} % draft of final

% Keywords command
\providecommand{\keywords}[1]
{
  \small
  \textbf{\textit{Keywords---}} #1
}

\usepackage[capitalise,noabbrev]{cleveref}
% \crefrangeformat{enumi}{#3#1#4-~#5#2#6}
% \crefformat{enumi}{#2#1#3}
% \crefrangeformat{equation}{#3#1#4-~#5#2#6}
% \crefformat{equation}{Equation #2#1#3}
% \crefformat{section}{Section #2#1#3}



